Casimir Effect in systems in and out of Equilibrium

This thesis consists on two separate parts. In the first part, we discuss about the nature of the Casimir effect as the response of a fluctuant medium to the breakdown of the translation symmetry because the presence of intrusions in that medium. To do so, we present a dynamical approximation of Casimir effect, which generalizes Casimir effect studies to out of equilibrium steady states. The equilibrium known case is recovered as a particular case, including the case of electromagnetic (EM) Casimir effect generated because of quantum fluctuations. This formalism also allows us to define (and calculate) the variance of Casimir forces. In the second part of this thesis, by the use of a Multiscattering formalism, we study the nature of the multibody Casimir effect. We demonstrate that the Casimir force and energy between two spheres in presence of a plate (perfect metal objects all of them) is non-monotonous with the distance between spheres and between sphere and plate. We derive the Pairwise Summation Approximation (PSA) of the EM field from this multiscattering formalism for generalized dielectrics, including magnetic responses and Topological Insulators as an example of magnetoelectric couplings. We also study the nonmonotonous behavior of the entropy with the temperature for a system of two perfect metal spheres and describes the Casimir energy between non-parallel cylinders, a geometry not studied until now to our knownledge.

==> Makefile <==
##################################################################
#
# LaTeX / PDFLaTeX Makefile
# (c) Tom Bobach 2007
# (c) Alexei Gilchrist 2008
#
# History:
#   24-09-2008  (AG) Stripped away some of the more dangerous code
#   17-07-2007  (TB) Added 2-levels of recursion for include checks
#   09-05-2007  (TB) Initial Version
#
# Disclaimer:
#   Use at your own risk.
#   I take no responsibility for this Makefile eating up your most
#   precious work, teaching your baby bad language or evoking evil
#   ghosts.
#
# What happens:
#   The current directory is searched for a *.tex file containing
#   the string "\documentclass"; this will be the main file.
#   All files included in the main file via "\include" will be
#   added to the source files.
#
#   If any of the input files contains the string "\bibliographystyle",
#   bibtex is invoked, the make dependency linked to the bib file found
#   in the "\bibliography{<file>}" entry.
#
# Usage:
#   make info        prints some info about the setup, what is considered
#                    the main file, what is the bibliography, what are
#                    the relevant images etc.
#   make clean       removes typical intermediate files.
#   make [pdf]       runs as stated in the beginning, assuming as target
#                    a pdf named after the main file.
#   make ps          like above, targeting a postscript
#   make dvi         like above, targeting a dvi
#   make view        opens kdvi with errors piped to /dev/null
#   make watch       checks every second for changes in *.tex, and *.bib
#
#
# TODO:
#   - support an arbitrary number of levels of recursion (currently 2)
#   - strip the comments from the texfile for every analysis of the text
#     (currently only done for bib file inclusion)
##################################################################

##################################################################
#   Main definitions - place your customizations here
##################################################################

MAINFILE=$(shell grep -l "\\\\documentclass" *.tex)

##################################################################
#   Some Definitions that should not need change
##################################################################

ifneq ($(words $(MAINFILE)),1)
$(error For automatic main file detection, only one .tex file can contain the "\documentclass" string. run make MAINFILE=<your mainfile>)
endif
# Currently, only two levels of recursion for included input is supported.
# If you need more, extend as you like after the scheme below.
TEXFILESPRE:=\
  $(shell grep "\\\\include{" $(MAINFILE) | sed 's/.*{\([^}]*\)}.*/\1/g') \
  $(shell egrep "\\\\input{.*}" $(MAINFILE) | sed 's/.*{\([^}]*\)}.*/\1/g')

ifneq ($(words $(TEXFILESPRE)),0)
  TEXFILES:=\
    $(MAINFILE:.tex=)\
    $(TEXFILESPRE)\
    $(shell grep "\\\\include{" $(TEXFILESPRE:=.tex) | sed 's/.*{\([^}]*\)}.*/\1/g') \
    $(shell egrep "\\\\input{.*}" $(TEXFILESPRE:=.tex) | sed 's/.*{\([^}]*\)}.*/\1/g')
else
  TEXFILES:=$(MAINFILE:.tex=) $(TEXFILESPRE)
endif


MUTE=@
SILENT=> /dev/null
VERYSILENT=1> /dev/null 2>/dev/null

MAKE=make --no-print-directory
LS=ls -1 --color=none
CP=cp

LATEX=pdflatex -shell-escape -interaction=nonstopmode
BIBTEX=bibtex

MSG_LAB_CHANGED="LaTeX Warning: Label(s) may have changed"
MSG_REF_UNDEFINED="LaTeX Warning: Reference.*undefined on input line.*"
MSG_CIT_UNDEFINED="LaTeX Warning: Citation.*undefined on input"

# strip all comments and extract the bibliography
FIND_BIB_FILE=$(shell \
	sed -e "s/\\\\%//g" $(1) | \
	sed -e "s/\([^%]*\).*/\1/g" | \
	grep "\\\\bibliography{"  | \
        sed 's/.*{\([^}^ ]*\)}.*/\1/g').bib

BIBFILE:=$(call FIND_BIB_FILE, $(TEXFILES:=.tex))
ifneq ($(BIBFILE),.bib)
  ifneq ($(wildcard *.bib),)
    BBL:=$(MAINFILE:.tex=.bbl)
  endif
endif


##################################################################
#   All the shell magic that helps us manage the twisted LaTeX
#   Compilation procedure
##################################################################


clear_valid=( [ ! -e .valid ] || $(RM) .valid )
check_undef_citations=\
  ( egrep $(MSG_CIT_UNDEFINED) $(MAINFILE:.tex=.log) > /dev/null )

# determine the changeset for citations
define check_citationchange
	(                                                \
	  [ -e .citations ] || touch .citations ;        \
	  ( grep "\\citation" $(MAINFILE:.tex=.aux)      \
		| sort                                   \
		| uniq                                   \
		| diff .citations -                      \
		> .citediff                              \
	  )                                              \
	)
endef

# exctract the citations from the aux file
define make_citations
	(                                                   \
	  (                                                 \
	    [ -e $(MAINFILE:.tex=.aux) ] &&                 \
	    ( echo "[info] Extracting citations...";        \
		grep "\\citation" $(MAINFILE:.tex=.aux)     \
		| sort                                      \
		| uniq                                      \
		> .citations                                \
	    )                                               \
	  )                                                 \
	  || touch .citations                               \
	)
endef

# comparing the citations in $(MAINFILE:.tex=.aux)
# against those in .citations.
# if there are differences, .citediff is changed.
define make_citediff
	(                                                     \
	  ( [ -e .citations ] || touch .citations ;           \
	    [ -e .citediff  ] || touch .citediff ;            \
	    echo "[info] Checking for changed Citations..." ; \
	    grep "\\citation" $(MAINFILE:.tex=.aux)           \
		| sort                                        \
		| uniq                                        \
		| diff .citations -                           \
	    > .citediff__                                     \
	  )                                                   \
	  || mv .citediff__ .citediff                         \
	)
endef

# compiles the document
# the file .valid is created if the compilation went without
# errors
define runtexonce
  ( 	                                                    \
    $(clear_valid);                                         \
    ( $(LATEX) $(MAINFILE) $(SILENT) &&                     \
      touch .valid );                                       \
    (                                                       \
      ( egrep $(MSG_REF_UNDEFINED) $(MAINFILE:.tex=.log)    \
        > .undefref ) ;                                     \
      ( egrep $(MSG_CIT_UNDEFINED) $(MAINFILE:.tex=.log)    \
        > .undefcit ) ;                                     \
      true                                                  \
    )                                                       \
  )
endef

# compile the document as many times as necessary to
# have cross-references right
define runtex
(                                                                      \
  echo "[info] Running tex...";                                        \
  $(runtexonce);                                                       \
  while( grep $(MSG_LAB_CHANGED) $(MAINFILE:.tex=.log) > /dev/null ) ; \
  do                                                                   \
      echo "[info] Rerunning tex...";                                  \
      $(runtexonce);                                                   \
  done                                                                 \
)
endef

##################################################################
#   Main compilation rules
##################################################################

pdf: $(MAINFILE:.tex=.pdf)

ps: $(MAINFILE:.tex=.dvi)

dvi: $(MAINFILE:.tex=.ps)



$(MAINFILE:.tex=.pdf): .compilesource
	$(MUTE)echo "[info] Created PDF."

# the dvi creation path invokes standard tex 
$(MAINFILE:.tex=.dvi): .force
	$(MUTE)$(MAKE) .compilesource \
		LATEX="latex -shell-escape -interaction=nonstopmode" 

%.ps: %.dvi
	$(MUTE)echo "[info] Converting DVI to PS"
	$(MUTE)dvips $< -o $@ $(VERYSILENT)

.compilesource: .force
	$(MUTE)$(MAKE) .valid
	$(MUTE)[ -z "$(BBL)" ] || $(MAKE) .citations
	$(MUTE)[ -e .valid ] || (                                    \
	  ( [ -e .compiled ] || $(MAKE) .compiled ) ;                \
	  ( [ -e .compiled ] || $(MAKE) .compiled ) ;                \
	  ( [ -e .compiled ] || $(MAKE) .compiled ) ;                \
	  ( [ -e .compiled ] || echo "[Error] Could not make it work after 3 runs. Weird." ) \
	)
	$(MUTE) (                                                    \
           echo ; echo "Compilation Warnings:" ;                     \
	   grep "Warning" $(MAINFILE:.tex=.log) ;                    \
	   grep "Error" $(MAINFILE:.tex=.log) ;                      \
	   grep -A 1 "Undefined" $(MAINFILE:.tex=.log) || true       \
	)
	$(MUTE)[ ! -e $(MAINFILE:.tex=.bbl) ] || (                   \
	  echo ; echo "Bibtex Warnings:" ;                           \
	  grep "Warning" $(MAINFILE:.tex=.blg) ;                     \
	  grep "Error" $(MAINFILE:.tex=.blg) || true                 \
	)
	$(MUTE)[ -z "$(BBL)" -a -e .valid ] || [ -n "$(BBL)" -a -e .compiled ]


clean:
	$(MUTE)$(RM) *.bbl *.blg *.aux *.log *.toc *.lof *.lot
	$(MUTE)$(RM) .??*


view: $(MAINFILE:.tex=.pdf)
	kpdf $< > /dev/null 2>&1 &

viewdvi: $(MAINFILE:.tex=.dvi)
	kdvi $(<:.dvi=) > /dev/null 2>&1 &

viewps: $(MAINFILE:.tex=.ps)
	kghostview $< > /dev/null 2>&1 &

info:
	@echo Main file:    $(MAINFILE)
	@echo Input files:  $(TEXFILES:=.tex)
	@echo Bibliography: $(BIBFILE)

# just do one run...
.valid: $(TEXFILES:=.tex)
	$(MUTE)$(runtex)

# if citations changed since last run of bibtex, run it again.
.citations: .citediff $(BIBFILE)
	$(MUTE)[ ! -e .compiled ] || rm .compiled
	$(MUTE)(                         \
	  echo "[info] Running BibTex" ; \
	  bibtex $(MAINFILE:.tex=) $(SILENT)         \
	) && $(make_citations)
	$(MUTE) $(clear_valid)

.citediff: .force
	$(MUTE)$(make_citediff)

# run as long as necessary
.compiled: $(TEXFILES:=.tex) $(BBL) 
	$(MUTE)echo "Found undefined Citations, rerunning..."
	$(MUTE)$(runtex)
	$(MUTE)$(check_undef_citations) || touch .compiled

.force:

define runwatch
  $(MUTE)CHANGE=true && while true ; \
  do       \
    if $$CHANGE ; then                             \
      echo;                             \
      echo "#######################################"; \
      echo "#    RUNNING MAKE                     #"; \
      echo "#######################################"; \
      echo;                                       \
      make;                                        \
      for i in $(TEXFILES:=*.tex) $(BIBFILE) ; do   \
        touch .$$i -r $$i;                         \
      done;                                        \
      CHANGE=false;                                \
    fi;                                            \
    sleep 2;                                       \
    echo 'tic' ; \
    for i in $(TEXFILES:=*.tex) $(BIBFILE) ; do     \
      if [ .$$i -ot $$i ] ; then                   \
        CHANGE=true;                               \
      fi                                           \
    done ;                                         \
  done
endef

watch:
	$(runwatch)


==> abstract.tex <==
\chapter{\OJO{Abstract}}

\section{English}

This thesis consists on two separate parts.

In the first part, we discuss about the nature of the Casimir effect as the response of a fluctuant medium to the breakdown of the translation symmetry because the presence of intrussions in that medium. To do so, we present a dynamical approximation of Casimir effect, which generalizes Casimir effect studies to out of equilibrium steady states. The equilibrium known case is recovered as a particular case, including the case of electromagnetic (EM) Casimir effect generated because of quantum fluctuations. This formalism also allows us to define (and calculate) the variance of Casimir forces.


In the second part of this thesis, by the use of a Multiscattering formalism, we study the nature of the multibody Casimir effect. We demonstrate that the Casimir force and energy between two spheres in presence of a plate (perfect metal objects all of them) is non--monotonous with the distance between spheres and between sphere and plate. We derive the Pairwise Summation Approximation (PSA) of the EM field from this multiscattering formalism for generalized dielectrics, including magnetic responses and magnetoelectric couplings. We also study the nonmonotonous behavior of the entropy with the temperature for a system of two perfect metal spheres and describes the Casimir energy between non--parallel cylinders, a geometry not studied until now to our knownledge.


\section{Español}
Esta tesis consta de dos partes diferenciadas.

En la primera parte, se realiza una discusión sobre la naturaleza del efecto Casimir como la respuesta de un medio fluctuante a la ruptura de la simetría de translación debido a la presencia de intrusiones en el mismo. Para desarrollar esta idea, presentamos una aproximación dinámica del efecto Casimir, que generaliza los estudios en efecto Casimir a estados estacionarios fuera del equilibrio. El caso conocido del equilibrio se recupera como un caso particular, incluyendo el caso de efecto Casimir electromagnético generado por fluctuaciones cuánticas. Este formalismo también nos permite definir y calcular la varianza de las fuerzas de Casimir.


En la segunda parte de la tesis, mediante el uso del formalismo de multiscattering, estudiamos la naturaleza de la interacción de Casimir en sistemas de varios cuerpos. Demostramos que la fuerza y la energía de Casimir entre dos esferas en presencia de una placa (siendo todos los objetos metales perfectos) es no monótona con la distancia entre las esferas y entre esfera y placa. También derivamos la Pairwise Summation Approximation del efecto Casimie elecromagnético a partir del formalismo de multiscattering para dieléctricos generalizados, incluyendo respuestas magnéticas y acoplos magneto-eléctricos. También estudiamos el comportamiento no monótono de la entropía con la temperatura para un sistema de dos esferas metálicas, aprovechando para explicar el sentido físico de dicha entropía negativa y, por último, obtenemos la energía de Casimir entre cilindros no paralelos, que es una geometría que no ha sido estudiada hasta ahora.



==> erratum.tex <==
\begin{savequote}[11cm] % this sets the width of the quote
\sffamily
``\textbf{Quotation}: \textit{n}. The act of repeating erroneously the words of another.''
\qauthor{Entry of The Devil's Dictionary, by Ambrose Gwinnett Bierce}
\end{savequote}

%\begin{savequote}[11cm] % this sets the width of the quote
%\sffamily
%``Oh Dear''
%\qauthor{Beatriz S\'anchez Garc\'ia, Private communication}
%\end{savequote}

\chapter{Erratum}
\graphicspath{{01-Casimir_Langevin/ch2/Figuras/}
{./01-Casimir_Langevin/ch2/Figuras}} 


Due to an inexplicable reason, in the printed version of this thesis, the Greek letter tau has been substituted by an empty space in all the formulas where it appeared, but just in the case when it appeared in normal size.


Next I give a list with the formulas where the tau's are skipped:


\begin{itemize}
\item Chap. \ref{Dynamical approach to the Casimir effect}:
\begin{itemize}
\item Sect. \ref{sec.2}: Eqs.~\eqref{solutionLangevin}.
\item Sect. \ref{Computation of Casimir forces}: Eqs.~\eqref{temporal-mode-evolution}, \eqref{two-field-modes-average} and \eqref{correlation.noise.modes}.%, \eqref{}, \eqref{}, \eqref{}, \eqref{}.
\item Appendix B, \ref{Apendice-Resolucion.promedio.modos.phi_n.phi_m}: Eqs.~\eqref{average-square-field2}, \eqref{correlation.noise.modes2}, \eqref{correlation.noise.modes3} and \eqref{correlation.noise.modes4}.
\item In the text next to Eq.~\eqref{correlation.noise.modes4}, $z_{1} = t - \tau_{1}$ and $z_{2} = t - \tau_{2}$.
\end{itemize}
\item Chap. \ref{Chap: Stochastic Quantization and Casimir forces.}:
\begin{itemize}
\item Sect. \ref{Parisi-Wu formalism}: Eqs.~\eqref{PW2}, \eqref{eq.Parisi-Wu}, \eqref{eq.noise}, \eqref{eq.phi} and \eqref{eq.eigenfunctions}.
\item In the text next to Eq.~\eqref{Pphi}, ($t = i\tau$).
\item In the text next to Eq.~\eqref{eq.Parisi-Wu}, $\phi(\tau,\textbf{r})\to \phi(\tau,\textbf{r};s)$.
\item In the text next to Eq.~\eqref{eq.eigenfunctions}, $g_{m}(\tau)$ and $g_{m}(\tau)=\exp(i\omega_m\tau)/\sqrt{\beta\hbar}$.
\item At the beginning of Sect. \ref{Casimir forces from the average stress tensor_PW}: $\eta(\tau,\textbf{r};s)$.
\item Sect. \ref{Perfect metal pistons of arbitrary cross section}, Fig. \ref{Figura_Piston_Circular}.
\item Appendix B, \ref{Appendix B: Derivation of the fluctuations of the force.}: Eqs.~\eqref{SDE_fluctuaciones}, \eqref{autocorrelacion_ruido_en_varianza}, \eqref{eigenproblem_varianza}, \eqref{eq.phiv2}, \eqref{4_points_correlation_function_definition}, \eqref{varianza_larga_2}, \eqref{4_points_correlation_function_result}, \eqref{4_points_correlation_function_result_12} and \eqref{4_points_correlation_function_result_2}.
\item In the text next to Eq.~\eqref{varianza_larga_3}, $\eta(i) = \eta(\textbf{r}_{i},\tau_{i},\sigma_{i})$.
\item In the text next to Eq.~\eqref{varianza_larga_4}, $\tilde{\delta}(i - j) = \delta(\textbf{r}_{i} - \textbf{r}_{j})\delta(\tau_{i} - \tau_{j})\delta(\sigma_{i} - \sigma_{j})$.
\item In the text next to Eq.~\eqref{4_points_correlation_function_result}, $\tau_{1} = \tau_{2} = \tau_{3} = \tau_{4} = \tau$, and $g_{m_{k}}(\tau)$.
%\item Sect. \ref{Computation of Casimir forces}: Eqs.~\eqref{temporal-mode-evolution}, \eqref{two-field-modes-average} and \eqref{correlation.noise.modes}.%, \eqref{}, \eqref{}, \eqref{}, \eqref{}.
%\item Appendix B, \ref{Apendice-Resolucion.promedio.modos.phi_n.phi_m}: Eqs.~\eqref{average-square-field2}, \eqref{correlation.noise.modes2}, \eqref{correlation.noise.modes3} and \eqref{correlation.noise.modes4}.
%\item In the text next to Eq.~\eqref{correlation.noise.modes4}, $z_{1} = t - \tau_{1}$ and $z_{2} = t - \tau_{2}$.
\end{itemize}
\end{itemize}


In addition, Figure \ref{Figura_Piston_Circular}, also inexplicably, has been incorrectly printed, it should appears as shown here:

\begin{figure}[htb]
\includegraphics[width=0.9\columnwidth,angle=0]{Figura_Piston.pdf}
\caption{Geometry of the perfect metal piston system, for the particular case of circular cross section. The the cavity and the piston are perfect metals. The piston is at a finite distance $L$ of one of the faces of the cavity, and at a distance $L_{\infty}$ of the other face. This distance tends to infinity in the calculations of the Chapter, but studies of finite $L_{\infty}$ are straightforward.}
\label{fig.plates}
\end{figure}




==> listofsymbols.tex <==
\chapter{List of Symbols}

% please change this list to suit your thesis

The following list is neither exhaustive nor exclusive, but may be helpful.
\begin{list}{}{%
\setlength{\labelwidth}{24mm}
\setlength{\leftmargin}{35mm}}
\item[$a$, $b$, $c$, $d$\dotfill] annihilation operators
\item[$a^\dagger$, $b^\dagger$, $c^\dagger$, $d^\dagger$\dotfill] creation
operators
\end{list}

